Space-Based Cosmic-Ray and Gamma-Ray Detectors: a Review

Prepared for the 2014 ISAPP summer school, this review is focused on space-borne and balloon-borne cosmic-ray and gamma-ray detectors. It is meant to introduce the fundamental concepts necessary to understand the instrument performance metrics, how they tie to the design choices and how they can be effectively used in sensitivity studies. While the write-up does not aim at being complete or exhaustive, it is largely self-contained in that related topics such as the basic physical processes governing the interaction of radiation with matter and the near-Earth environment are briefly reviewed.

==> sec_future.tex <==
\section{Future Developments}


\fixme{Near future: DAMPE and CALET.}


\fixme{Mid term: Gamma-400 and HERD.}


\fixme{ISS-CREAM?}

